Adapt PointFormer: 3D Point Cloud Analysis via Adapting 2D Visual Transformers

Pre-trained large-scale models have exhibited remarkable efficacy in computer vision, particularly for 2D image analysis. However, when it comes to 3D point clouds, the constrained accessibility of data, in contrast to the vast repositories of images, poses a challenge for the development of 3D pre-trained models. This paper therefore attempts to directly leverage pre-trained models with 2D prior knowledge to accomplish the tasks for 3D point cloud analysis. Accordingly, we propose the Adaptive PointFormer (APF), which fine-tunes pre-trained 2D models with only a modest number of parameters to directly process point clouds, obviating the need for mapping to images. Specifically, we convert raw point clouds into point embeddings for aligning dimensions with image tokens. Given the inherent disorder in point clouds, in contrast to the structured nature of images, we then sequence the point embeddings to optimize the utilization of 2D attention priors. To calibrate attention across 3D and 2D domains and reduce computational overhead, a trainable PointFormer with a limited number of parameters is subsequently concatenated to a frozen pre-trained image model. Extensive experiments on various benchmarks demonstrate the effectiveness of the proposed APF. The source code and more details are available at https://vcc.tech/research/2024/PointFormer.

==> sec/6_more_analysis.tex <==
\section{Limition and Future Work}
\textbf{Limition.}

\noindent Although the APF method has shown promising results in terms of effectiveness, its performance improvements come with a trade-off. When compared to existing methods that fine-tune 2D pre-trained models, APF requires an increase in the number of training parameters.   Despite these drawbacks, the performance gains offered by APF suggest potential benefits in scenarios where high accuracy is critical and resources are less of a constraint. Future research could explore ways to optimize the number of parameters without significantly compromising the method's effectiveness, potentially broadening the applicability of APF in practical settings.

\noindent\textbf{Future Work.}

\noindent During the research process, we find RPN(Random PointNet) embedding without training can also attain a comparable results in classification.this can also prove that \textbf{Our method's effectiveness is not depend on light weight PointNet but actually the pre-train ViT model}.Thus, we might ask \textit{Can a standard ViT serve as a general backbone for point cloud analysis, rather than using diverse backbones?}
This will be a research focus for improvement in our future work.


\noindent During our research, we discovered that employing RPN (Random PointNet) embeddings without any training can still achieve comparable results in classification tasks.This finding underscores that \textbf{the success of our approach does not rely solely on the lightweight PointNet architecture.} Instead, it appears that the significant contributory factor is the pre-trained ViT (Vision Transformer) model. Consequently, this leads us to consider \textit{whether a standard ViT could be effectively used as a universal backbone for point cloud analysis, instead of relying on a variety of specialized backbones.}

\noindent Given this context, our future research will focus on exploring the potential of the ViT model as a general backbone in point cloud analysis. We aim to conduct extensive experiments to compare the efficacy of ViT against other common backbones in handling various point cloud-related tasks. This will help us to better understand the capabilities and limitations of using ViT in diverse application scenarios, potentially leading to significant advancements in the field.


==> tab/part_res_cls.tex <==
\begin{table}[tb]
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 \centering  % 显示位置为中间
 \caption{Comparison results.} 
 \label{tab:cls_res}
 %\setlength{\tabcolsep}{15pt}
 \resizebox{1\linewidth}{!}  
 %\renewcommand{\arraystretch}{0.9}
{\begin{tabular}{c|c|c|c}
  \toprule
  Methods & pointnet & pointmlp & pointnet* \\ \hline
  scanobjectnn(hardest) & 83.1 & 87.8 & 79.4 \\ \hline
  scanobject(easy) & ? & - & - \\ \hline
  scanobject(easy-background) & ? & - & - \\ \hline 
  modelnet40 & 94.15 & ? & 91.1\\ \hline
  shapenetpart & ?  & - &  - \\ 
  \bottomrule
  \end{tabular}}
\end{table}



pointnet=pointnet+vit+sort \\
pointmlp=pointmlp+vit \\
pointnet*=freeze encoder=sort+adaptformer \\
?=soon to run\\
- = no run 

